The trans- and post-capture orbital evolution of Triton

Triton is a unique moon in our Solar System, being the only large moon to orbit on a retrograde and highly inclined orbit. As a result, it is thought that it did not form around Neptune, but rather was captured from heliocentric orbit. The resulting tidal heating is likely to have been sufficient to melt Triton's mantle several times over. Previous work on the topic has required simplifying assumptions or application of mathematical methods outside of the domain in which they are well-behaved. In this work, we revisit the description of this period of Triton's history, by developing methods that allow us to simulate high-eccentricity spin-orbit evolution for an arbitrary rheological model. Our aim is to provide a framework on which future work can build with more detailed planetological models, while still capturing the full intricacies of high-eccentricity tidal evolution. We forego simplifications used in past work and rather determine the convergence properties of each infinite sum in the Darwin-Kaula expansion, truncating them appropriately. We achieve this with a new conservative empirical upper bound on the expansion into eccentricity functions of part of the tidal potential, and with a novel, fast-converging power series expansion for these eccentricity functions borrowed from artificial satellite theory. Consequently, we examine the case of Triton. We find that the use of the constant time lag model fails to match the capture into spin-orbit resonances we expect from a sufficiently viscous icy body at non-zero eccentricities. Additionally, we find that Triton can have experienced tidal heating rates orders of magnitude greater even than present-day Io, and so likely possessed a massive Titan-like atmosphere throughout its tidal evolution, with a surface or thin-shell ocean. Whether this would significantly extend the epoch of tidal heating will be the subject of future work.

==> frontmatter/nomenclature.tex <==
% Put acronyms, units and constants in 1 chapter

\chapter{Nomenclature}
\label{front:nomenclature}

% print acronyms (only the ones that are refered to in the text)
\printglossary[type=acronym, style=long-name-desc-loc]

\renewcommand*{\glsgroupskip}{} % no vertical indent for each new group, doesnt seem to work, hence all constants start with c: and all units start with u:

\printglossary[type=constants, style=long-name-desc-sym] % adding constants is optional
\printglossary[type=units, style=long-name-desc-sym] % adding units is optional

% Add all constants and units to the tables
\glsaddall[types=constants] % optional
\glsaddall[types=units] % optional

